Attention-guided Generative Models for Extractive Question Answering

We propose a novel method for applying Transformer models to extractive question answering (QA) tasks. Recently, pretrained generative sequence-to-sequence (seq2seq) models have achieved great success in question answering. Contributing to the success of these models are internal attention mechanisms such as cross-attention. We propose a simple strategy to obtain an extractive answer span from the generative model by leveraging the decoder cross-attention patterns. Viewing cross-attention as an architectural prior, we apply joint training to further improve QA performance. Empirical results show that on open-domain question answering datasets like NaturalQuestions and TriviaQA, our method approaches state-of-the-art performance on both generative and extractive inference, all while using much fewer parameters. Furthermore, this strategy allows us to perform hallucination-free inference while conferring significant improvements to the model's ability to rerank relevant passages.

==> tables/backoff.tex <==

\begin{table}[h!]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize

\begin{tabu}{@{}lcc@{}}
\toprule
 &  \multicolumn{2}{c}{\textsc{TriviaQA}} \\
 &  \multicolumn{2}{c}{\textsc{Best Result}} \\
\cmidrule(r){2-3}
\textbf{Model} & EM & F1 \\
\midrule
BART-large & - & - \\
+ drop & - & - \\
+ naive & - & - \\
+ oracle & - & - \\


\bottomrule
\end{tabu}
\end{minipage}
\caption{Comparing various versions of back-off. Naive ensures no hallucination while more intelligent methods can further improve the state-of-the-art model.}
\label{table:backoff}
\end{table}

==> tables/constrained.tex <==

\begin{table}[h!]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize

\begin{tabu}{@{}lcccc@{}}
\toprule
 &  \multicolumn{4}{c}{\textsc{Natural Questions}} \\
  &  \multicolumn{2}{c}{\textsc{Abstractive}} & \multicolumn{2}{c}{\textsc{Extractive}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} 
\textbf{Model} & EM & F1 & EM & F1 \\
\midrule
BART-large & 52.58 & 60.30 & 35.15 & 47.65 \\
BART-large + constr. & 46.48 & 56.30 & 32.66 & 45.77 \\
BART-large + joint & 53.43 & 60.76 & 50.03 & 58.27 \\


\bottomrule
\end{tabu}
\end{minipage}
\caption{Results on Natural Questions shows that our method outperforms other baselines. Constrained decoding forces the vocabulary to be in-context during inference.}
\label{table:constrained}
\end{table}



==> tables/in_passage.tex <==
\begin{table}[h!]
\begin{minipage}{1.0\linewidth}
	\centering
	\footnotesize

\begin{tabu}{@{}lcc@{}}
\toprule
  &  \multicolumn{2}{c}{\textsc{Hallucination (in percent)}} \\
\textbf{Model} & total & improper \\
\midrule
Natural Questions & 9.11 & 5.26 \\
TriviaQA & 21.94 & 6.96 \\

\bottomrule
\end{tabu}
\end{minipage}
\caption{The percent of improper hallucinations corresponds to the hallucinations where the generated prediction is not found, but the ground truth answer is found, in the retrieved context. The FID model we trained exhibits significant amounts of hallucination, over half of which are improper.}
\label{table:in_passage}
\end{table}


